Design Challenges for Reconnecting in Later Life: A Qualitative Study

Friendships and social interactions are renown contributors to wellbeing. As such, keeping a healthy amount of relationships becomes very important as people age and the size of their social network tends to decrease. In this paper, we take a step back and explore reconnection -- find out about or re-contact old friends, an emerging topic due to the increased use of computer-mediated technology by older adults to maintain friendships and form new ones. We report on our findings from semi-structured interviews with 28 individuals from Costa Rica and Poland. The interviews aimed to explore whether there is a wish to reconnect, and the challenges encountered by older adults to reconnect. We contribute with design considerations for tools allow- ing older adults to reconnect, discussing opportunities for technology.

==> sections/results.tex <==
\section{Results}


%\subsection{Participants}

%Poland - In 8 of 11 interviews respondents bring photos with POI. 
%Paraguay - Every respondent provided us picture to talk about. 

\subsection{Characterizing the person of interest}
Former relationships between participants and POIs can be categorized into: classmates, colleagues, friends, neighbors, and others. In Costa Rica the relationships were more varied, participants indicated colleagues (7), friends (4), neighbors (2), classmates (1), band members (2) and priests from their neighborhood (2). Most participants from Poland did not reveal the relationship with the POI, but those who did, reported classmates (6), friends (2), and neighbors (1).
%\textbf{xxx perhaps also for the below we can summarize results in a table, where the rows (or cols) are the classes of questions or the individual questions, and cols are the 3 study locations, and in the cell we put a summary of the findings for that questions and location? this makes sense if we can summarize the results and fit them in a cell}

%Some of the participants were spontaneously giving information about the POIs, most notably about their character (9; e.g. ``was nice to me'', ``was cheerful'', ``was gentle and humble'') and activities together (4; e.g. `` ... used to meet for coffee'', ``used to invite me for praying'').

When describing the POI, some participants from Costa Rica (9) were spontaneously giving information about the character of the POI. On the other hand,  participants from Poland (5) talked about the POIs' jobs, families or hobbies.

\begin{table}
  %\centering
  %\begin{tabular}{l p{1.2cm} p{1.2cm} p{1.2cm} p{1cm}}
  \begin{tabular}{p{2cm} p{2.8cm} p{2.8cm} }
    % \toprule
    {\small\textit{Characteristic}}
    & {\small \textit{Costa Rica (n=18)}}
      %& {\small \textit{Paraguay (n=5)}}
      & {\small \textit{Poland (n=11)}} \\
      %& {\small \textit{All (n=34)}}\\
    \midrule
    Relationship with POI & 7 colleagues, 4 friends, 2 neighbors, 1 classmate, 2 band members, 2 priests 
                        %& 3 classmates, 1 colleague, 1 member of political party
                        & 6 classmates, 2 friends, 1 neighbor, 2 relationship not disclosed \\
                        %& 10 classmates, 8 colleagues, 6 friends, 3 neighbors, 5 others \\
    
    Friends in common & 6 three or more, 4 two, 5 one, 3 none 
                             %& 4 three or more, 1 none 
                             & 10 three or more, 1 one \\
                             %& 20 three or more, 4 two, 6 one, 4 none\\
    %\bottomrule
     % All & 34 & 65 & & 
  \end{tabular}
  \caption{Characteristics of relationships between participants and POIs}~\label{tab:table2}
\end{table}

%\begin{table}
%  \centering
%  \begin{tabular}{l r r r r r}
%    % \toprule
%    {\small\textit{Location}}
%    & {\small \textit{Classmate}}
%    & {\small \textit{Colleague}}
%    & {\small \textit{Friend}} 
%    & {\small \textit{Neighbor}}
%    & {\small \textit{Other}} \\
%    \midrule
%    Costa Rica & 1 & 7 & 4 & 2 & 4 \\
%    Paraguay & 3 & 1 & 0 & 0 & 1 \\
%    Poland & 6 & 0 & 2 & 1 & 2 \\
%    \bottomrule
%     All & 10 & 8 & 6 & 3 & 7 \\
%  \end{tabular}
%  \caption{Former relationships between participants and POIs.}~\label{tab:table2}
%\end{table}

%Participants were also asked whether they could name up to three friends in common with the POI. In Paraguay and Poland almost all participants could name three friends in common (1 participant from Poland mentioned only one friend and 1 participant from Paraguay did not mention anyone), while in Costa Rica the responses distributed more evenly among three friends (6), two friends (4), one friend (5), and no friend at all (3).

%To assess whether the size of the social network had and effect on the chance to reconnect, 
To have a measure of the potential friends they could use as proxies to reconnect with the POI, we asked participants to name up to three friends in common. In Paraguay and Poland almost all participants could name three friends in common (1 participant from Poland mentioned only one friend and 1 participant from Paraguay did not mention anyone), while in Costa Rica the responses were distributed more evenly among three common friends (6), two friends (4), one friend (5), and no common friend at all (3).

%We discovered mobility to be quite different among our study locations. When we asked about \emph{where the POIs came from}, 
We also wanted to characterize the geographical separation, so we asked participants about the origin of the POIs. Participants from Costa Rica provided the most diverse responses. The majority of POIs were from Costa Rica (12), followed by Nicaragua (3), El Salvador (2) and Spain (1). In some cases, this happened because participants had moved from their country of origin, Nicaragua (2) and El Salvador (1), where they had met the POIs. Even within Costa Rica, the POIs were all from  outside Los Guido. Participants from Poland only named POIs from their own country,mostly from the same city where the interviews were conducted (5), or a larger city that was close and where many of the participants had attended university. The rest were from other cities in Poland (4).

These numbers show us that geographical distance, potentially due to relocation, is a common theme.

%geographical distribution
% participants' origin: Costa Rica (15), Nicaragua (2), El Salvador (1)
%POIs' origin: Costa Rica (12), Nicaragua (3), El Salvador (2), Europe/Spain (1)

\subsection{Loss of contact}
%reasons for losing contact
%Interviewee moved (9), POI moving (4), Leaving work (2), Others (3): POI got married, jealous husband, personal issues; no way to contact (+2)
Moving was revealed to be one of the main reasons for losing contact: 

``\emph{We were very good friends, but I did not see her again since I moved. We completely lost contact}'' (FC, 69F).

Most participants from Costa Rica lost contact after them or the POI moved (13). 
%including all of those who moved from their country of origin (3); when the POI moved (5, in 2 cases along with the participant moving) participants also lost contact. 
Some participants decided to end the relationship (3) because of personal issues, after the POI got married, and at the request of the participant's partner (along with the participant moving). Leaving work (3, in one case along with the participant moving) was another reason for lost contact.
In Poland too, the main reason to lose contact was the participant or the POI moving (6). Participants also reported losing contact when the association (e.g. work, school) with the POI ended (4, in 2 cases along with moving). Other reasons to lose contact were being busy (2) and ending the relationship because of an argument (1).

%\begin{table}
%  \centering
%  \begin{tabular}{l p{0.75cm} p{0.75cm} p{1.1cm} p{1.25cm} p{0.65cm}}
%    % \toprule
%    {\small\textit{Location}}
%    & {\small \textit{Moved}}
%    & {\small \textit{POI moved}}
%    & {\small \textit{No way to contact}} 
%    & {\small \textit{Association ended}}
%    & {\small \textit{Other}} \\
%    \midrule
%    Costa Rica & 9 & 4 & 2 & 2 & 3 \\
%    Paraguay & 0 & 0 & 0 & 3 & 3 \\
%    Poland & 1 & 5 & 2 & 4 & 3 \\
%    \bottomrule
%     All & 10 & 9 & 4 & 9 & 9 \\
%  \end{tabular}
%  \caption{Reasons to lose contact.}~\label{tab:table3}
%\end{table}
    

\subsection{Reconnection attempts}

In order to understand reconnection attempts, and to identify barriers and emerging scenarios for reconnection, we started by asking participants whether they have tried to reconnect with the POI. We considered valid reconnection attempts both inquiring about a POI or trying to contact the POI directly. 


Overall, 21 participants did not make an attempt to reconnect, 12 participants tried reconnecting with the POI either by trying to contact them directly (6) or by trying to find out about them (6). We even identified a successful reconnection case. Despite recent contact being a criterion for exclusion, we still proceeded with the interview since the participant had only recently resumed contact with the POI and we were interested in how the reconnection occurred. The participant told that a few days before our interviews she was reached by a friend and former colleague who was trying to organize a reunion. This friend had been able to trace back other former colleagues and created a group in Whatsapp. The participant was invited to join and she found the POI there: 

\textit{``[The POI] was there [in the Whatsapp group] and I added her to my Whatsapp contacts. Not only Whatsapp but Facebook too! Because I use Facebook on the phone''} (VM, 69F).

Breaking down the overall numbers by location we observe that in Paraguay none of the participants tried, while in Poland only 3 out of 11 participants made an attempt to reconnect either by trying to contact the POI (2) or to find out (1). In Costa Rica, half of the participants said they did not try (9) and the other half said they tried to contact (3) or find out about the POI (5): 

\textit{``I asked [friend in common] who is in contact [with POI]. Back then I had no cellphone or anything, so I did not ask for a number. Now I could ask, it’s easier to be connected to people''} (BB, 76F). 

\subsubsection{Participants with no reconnection attempts}
Perhaps the most interesting results come from our analysis on the reasons why the 21 participants did not try to reconnect. When we asked participants \textit{why}, only (6) participants said that they were not interested. In Poland, two participants stated no interest to reconnect. In Costa Rica one participant said she has an aloof personality and another participant reported not trying because of personal issues. Similarly, in Paraguay, one participant also reported personal issues as the reason for not trying to reconnect and one participant reported that the interest to reconnect had faded. 

 \textit{``[POI] was very shy and not very talkative, after [the end of] school each took different paths and one just starts losing interest''} (AA, 65F). 

The remaining 15 participants were potentially interested in reconnecting. Participants reported not trying because they had no way to contact the POI (6), they lived too far away (4), making an attempt to reconnect would have been awkward or inappropriate (3), and being busy (2). Interestingly, one of the participants in Poland said she was actively trying to reconnect at the time \textit{``I am about to [recontact]... via friends, I will call her friends [to get the contact]''} (ZO, 67F). In Paraguay one participant said there was no reason in particular for not trying. 

\subsubsection{Participants with reconnection attempts}
The reconnection cases include six attempts to contact the POI directly and other six finding out about the POI. In Costa Rica, five participants tried to find out and four tried to contact the POI while in Poland there was one attempt to find out and two attempts to contact the POI. No participant tried to reconnect in Paraguay.

In Costa Rica, when attempting to contact the POI directly, participants tried: calling the POI (2), visiting the POI (2) or a POI's relative (1), and even trying to reach the POI through a radio program that they used to listen together (1); when inquiring about the POI, participants tried asking someone in common: a relative (2), an acquaintance (2) or a friend (2) 
In Poland participants tried to contact the POI by calling the POI directly (2), and when inquiring about the POI by asking friends and acquaintances (1):

 \textit{``I wanted to establish contact [with the POI] so I asked friends from school but they did not know anything about [the POI]''} (KR, 69F). 

Nonetheless, these attempts did not lead to a successful reconnection. Overall, the most common reasons for which these attempts failed were not having a way to contact the POI (5) or losing track of the POI (4). 
In other cases the motivation faded when participants were only getting updates through friends in common (2) or after the POI did not reciprocate contact (1):  

 \textit{``We exchanged phone numbers... I tried to call two times, but [POI] did not responded nor called back... and contact was lost, i do not know why''} (JE, 68M)

\subsubsection{Facilitators of the reconnection}
Regarding potential helpers in the reconnection process, participants mentioned friends, family members, people close to the POI, acquaintances. Only 8 out of 33 participants could not think of anyone who could help. 

Interestingly, some participants mentioned that class reunions were events that they were looking forward to assist but complained that this events were not organized frequently enough. This was the case especially in Poland (4). Not to mention that the successful reconnection case previously mentioned came to happen because of a friend organizing a reunion.


%most participants from Costa Rica said they could not think of someone who could help (7), but others mentioned family members (1) and people close to the POI (5), such as friends in common (2), neighbors (2), or relatives (1). In Paraguay, participants reported that they would ask friends in common (3) and acquaintances (1). In Poland, most people said that they would ask friends (4) and family (3) for help. Other participants mentioned POI relatives (2) and not being able to think of anyone who could help (1). 




%Some participants were excluded from this analysis, including the successful reconnect case and one participant that reported having no interest (both form Costa Rica). The remaining participants were excluded because they all had a way to contact POIs. These include participants from Costa Rica (4) who reported not trying to reconnect to avoid problems with their partners or due to personal issues with the POI, one participant who said she was updated by a friend, and one participant who say would call the POI if going back to their country of origin. In Paraguay a participant had not called because of personal issues and In Poland a participant reported being too busy and that the POI live too far away.

%\begin{table}
%  \centering
%  \begin{tabular}{l r r r}
%    % \toprule
%    {\small\textit{Location}}
%    & {\small \textit{No attempt}}
%    & {\small \textit{Find out}}
%      & {\small \textit{Re-contact}} \\
%    \midrule
%    Costa Rica* & 9 & 3 & 5 \\
%    Paraguay & 5 & 0 & 0 \\
%    Poland & 8 & 1 & 2\\
%    \bottomrule
%     All & 22 & 4 & 7
%  \end{tabular}
%  \caption{Reconnection attempts. (*) The successful reconnection case is not accounted for in Costa Rica}~\label{tab:table4}
%\end{table}


%\begin{table}
%  \centering
%  \begin{tabular}{l p{1cm} p{1.25cm} p{1.25cm} p{1.25cm} p{0.65cm}}
%    % \toprule
%    {\small\textit{Location}}
%    & {\small \textit{Distance}}
%    & {\small \textit{No way to contact}}
%    & {\small \textit{No interest}}
%    & {\small \textit{Other}} \\
%    \midrule
%    Costa Rica & 4 & 3 & 1 & 5 \\
%    Paraguay & 0 & 2 & 2 & 1 \\
%    Poland & 3 & 2 & 2 & 2 \\
%    \bottomrule
%     All & 7 & 7 & 5 & 8 \\
%  \end{tabular}
%  \caption{Reasons for not trying to reconnect.}~\label{tab:table5}
%\end{table}

%To understand strategies for reconnection, we asked to participant how did they try to reconnect and who could help them to reconnect with the POI they selected.



%\textcolor{red}{discuss reasons for fail attempts to reconnect}

%\begin{table}
%  \centering
%  \begin{tabular}{l p{0.7cm} p{0.7cm} p{1cm} p{0.8cm} p{0.8cm} p{0.5cm}}
%    % \toprule
%    {\small\textit{Location}}
%    & {\small \textit{Family}}
%    & {\small \textit{Friend}}
%    & {\small \textit{Friend in common}}
%    & {\small \textit{Close to POI}} 
%    & {\small \textit{No one}}
%    & {\small \textit{Other}} \\
%    \midrule
%    Costa Rica & 1 & 0 & 2 & 3 & 7 & 0 \\
%    Paraguay & 0 & 0 & 3 & 0 & 0 & 1 \\
%    Poland & 3 & 4 & 0 & 2 & 1 & 0 \\
%    \bottomrule
%     All & 4 & 4 & 5 & 8 & 8 & 1 \\
%  \end{tabular}
%  \caption{Potential helpers to reconnect. This analysis excludes 8 participants}~\label{tab:table6}
%\end{table}

%\textcolor{red}{discuss willingness to reconnect}

 %{\color{blue} There were also some interesting cases of declared willingness or lack interests in recontact in Poland. Only (2) participant declared no interest of recontact. In (1) more due to distance, participant also lost interest in contacting POI: \textit{"i did not [tried to contact] because i never were going there [to POI city]}".  As already stated (3) were trying, so they were actively interested in contact. In addition (2) were directly declaring willingness to recontact POI as soon as possible - in one case participant was "about to": \textit{"I am about to [recontact]  (..) via friends, i will call her friends [to contact POI] "} and in other, participant had business card "with hope to contact soon":\textit{ "I do not know if i still have her [POI] business card... [participant is looking into wallet] ...oh, i have! [show card] (..) so i theoretically have contact, but not practically "  - "so you see, i hold it with hope to contact someday"}. 
 
 %In (2) cases participants mentioned cultural or social barrier with contacting POI. In one case it was about having spouses and families (in case of female friend for a man): \textit{"[About recontact attempts] We saw each other one or two times... but not close, not alone [suggesting that it would be inappropriate to meet alone] (..) she had husband, friend of mine and i also had my family so... (..) not close, always in group"  } in the other about awkwardness of engaging other people into recontact process: \textit{"We exchanged phone numbers... I tried to call two times, he did not responded nor called back... and contact was lost, i do not know why. In fact i could try to reach [POI], my daughter in law sister is working in [POI work], but i do not want to involve other people into this"}. 
 
 %In (2) more cases with reason like "no phone number" or "no one to ask" we could assume that if they had this possibility they could try. Even if we do not know that for sure, we could possibly make such opportunity.
 %}

%\subsection{Picture information}

%%picture context
%%unclassified 
%% - work out in class [group activity]
%% - work regular day  [regular day]
%% - no picture (3)
%% - trip (2)
%% - praying meeting (religious activity) [special event] [group activity]
%% - baptism of participant (religious activity) [life event]
%% - baptism of participant's daughter (reli act) [life event]
%% - farewell mass (rel act) [special event]
%% - lunch in festival (special event)
%% - school regular day [regular day]
%% - band playing in party (special event?) [special event]
%% - new year party [special event]
%% - work regular day [regular day]
%% - regular day [regular day]
%% - visiting POI regular day [regular day]

%%dates and places remembered
%Regarding picture information, in general, participants remembered little about \textit{when} the picture was taken. Eleven participants were able to provide imprecise information about the year
%% look for an actual quote, this is just a made up example
%(``It was about 5 or 6 years ago'') 
%and most participants did not remember the month (9) or day (7) at all. Interestingly, some participants did remember the time (5, when asked) and the time of the day (9, when asked) 
%%time of day probably easy to guess from the picture, for example if its outdoors
%, and could also relate the date to a close event (4, spontaneously; 5, when asked) 
%% again easy to tell from the picture what event it was

%For information on \textit{where} the picture was taken, many participants could remember the place (7, spontaneously; 3, when asked) or its name (4, spontaneously; 10, when asked). 
%% (e.g. the church, Plaza Viquez)
%But, much like with the POI, they had trouble connecting this place to a precise location such as the city or province. Again, this because they were not so aware of the political division. In addition, not a single participant was able to provide the address for the picture (10, no information; 5 we did not ask) \textbf{xxx what does it mean no info and not asked?}

%%pictures showing last contact, last meeting remembered, comparison with picture
%Only one participant brought a picture that portrayed the last meeting with the POI, while three brought pictures that did not include the POI. Nonetheless, we asked all participants (18) whether they remembered the last contact with the POI. Most participants could provide some information about the last meeting (6, spontaneously; 5 when asked) 
%%insert quote with example of what participants said

%Moreover, similarly to picture information, participants provided information about the time of the day (11, when asked) and on close events (5, spontaneously; 4, when asked). It is worth mentioning that most participants could not provide any information about the month (10) and day (9) of the last meeting.

%%

%Pictures with POI were all related to work or studies. One was picture of students celebrating end of college (near school), two was conference and science meetings, one was office barbecue party and only one not related to work (birthday party). 

%Almost all (4 of 5) remembered year and month when picture was taken. In 2 interviews they remembered exact date (and one even time). All places were picture was taken were recognized along with exact address. 

%Only in one case picture was showing last contact with POI. In interviews respondents generally could not remember a lot about last meeting. Only one could provide exact year. This is interesting contradiction to situation with picture, were a lot of information were provided. 

%%

%Technology probably could help with recontacting to first group. As it was almost half of our interviews and majority of people who did not tried to contact, this shows potential usefulness of technology in helping elderly people to recontact. 

%9 of 11 people bring photo and 8 was with POI on it. In most cases they bring a lot of picture and wanted to talk about them and picking one was hard task. Photos were very different: wedding, banquet, student festival, break in school (2 cases), warship, sport event, Christmas party at work and travel.

%Respondents usually remembered (mostly after some time to calculate) year when picture was taken, but none could remember exact date with day etc. They could, however, remember estimated hour or daytime of event. Context of photo was in all cases given spontaneously. They also usually remembered the place.

%Other people in pictures were usually known. In most cases they know some people (4 cases) from pictures or all (4 cases). Only in one case respondent did not know anyone from picture. However, only in 3 cases respondent was still in contact with some people from picture (in one case with all). In one case, at this point, respondent remembered that she actually found contact to POI once by other person from photograph. 

%Pictures were not usually last situation when respondents meet with POI. In 4 cases there were end of school, graduate or prom party after it. In 2 cases there were some kind of school or work reunion and in two cases respondent have meet with POI at birthdays parties of friend or family. 
